From Values to Opinions: Predicting Human Behaviors and Stances Using Value-Injected Large Language Models

Being able to predict people's opinions on issues and behaviors in realistic scenarios can be helpful in various domains, such as politics and marketing. However, conducting large-scale surveys like the European Social Survey to solicit people's opinions on individual issues can incur prohibitive costs. Leveraging prior research showing influence of core human values on individual decisions and actions, we propose to use value-injected large language models (LLM) to predict opinions and behaviors. To this end, we present Value Injection Method (VIM), a collection of two methods -- argument generation and question answering -- designed to inject targeted value distributions into LLMs via fine-tuning. We then conduct a series of experiments on four tasks to test the effectiveness of VIM and the possibility of using value-injected LLMs to predict opinions and behaviors of people. We find that LLMs value-injected with variations of VIM substantially outperform the baselines. Also, the results suggest that opinions and behaviors can be better predicted using value-injected LLMs than the baseline approaches.

==> 4-2-Training.tex <==

% In this section, we evaluate the LLMs understanding of the target value distribution and its ability to predict human behavior through following four experiments.
% In this section, we compare \villm~with baselines to demonstrate its ability of understanding values in four aspects.
% \todo{I think this subsection can be deleted along with Table~\ref{tab:experiments}. The content is redundant, and there is no appropriate section for them since the experiments are now split into 2 sections.} 
LLMs that have successfully been injected with certain value distribution should be able to reflect the value distribution consistently in various scenarios and tasks, such as, answering a value survey, making arguments, deciding actions in daily situations, and expressing political/religious stances.

We compare \villm~with baselines to demonstrate its ability of following tasks.
Section \ref{4-2-1-PVQ} describes how well the LLM responds to questions directly related to values through PVQ.
Section \ref{4-2-2-ArgGen} shows the ability of \villm~and in-context learning methods to generate value-related arguments by human evaluation.
In section \ref{4-2-3-VALUENET}, we evaluate whether LLM can predict human behavior in daily situations.
And finally, section \ref{4-2-4-ESS} explains LLMs ability to express stances on specific issues such as political and religious topics.
% Table \ref{tab:experiments} shows the summary of each experiment in terms of settings.
% The prompts used for each task are described in the Appendix \ref{appdx:prompts}. => 테이블에서 언급할 것입니다.

% In this section, we investigate value injected models are capable of predicting responses to real-world issues and predicting behavior in everyday life scenarios. 
% More recently, studies have focused on examining how people respond to political decisions such as voting, based on their prioritized values (\citealp{sagiv2000value}).






% \begin{table*}[t]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{llllll}
% \toprule
% Section & Dataset & Prompt & Model Output & Ground Truth & Metric  \\
% % \multicolumn{1}{c}{\textbf{Section}} & \multicolumn{1}{c}{\textbf{Dataset}} & \multicolumn{1}{c}{\textbf{Prompt}}                                 & \multicolumn{1}{c}{\textbf{Model Output}} & \multicolumn{1}{c}{\textbf{Ground Truth}} & \multicolumn{1}{c}{\textbf{Metric}}  \\
% \midrule
% \cref{4-2-1-PVQ}                                  & Portrait Values Questionnaire                                   & Table \ref{tab:APP_EXP_pvq_prompt} & Number                                    & Group value distribution                  & NMSE                                                                                        \\
% \cref{4-2-2-ArgGen}                                  & Touché23-ValueEval                          & Table \ref{tab:APP_EXP_AG_prompt} & Premise \& Stance                           & -                                        & Winning ratio                                                                           \\
% \cref{4-2-3-VALUENET}                                  & VALUENET                             & Table \ref{tab:APP_EXP_valuenet_prompt}                                                            & Agree or Disagree                                 & Group value distribution                  & NMSE                                                                                       \\
% \cref{4-2-4-ESS}                                  & European Social Survey                                  & Table \ref{tab:APP_EXP_ess_prompt}                                                                 & Number                                    & Number                                    & NMSE                                                  
% \\ 
% \bottomrule
% \end{tabular}}
% \caption{
% Summary of experiments to demonstrate that \villm~has the ability of reflecting the value distribution consistently in various tasks.
% `-' denotes the absence of ground-truth data, so we conduct a human evaluation where annotators determine the more appropriate generated argument between two different trained LLMs.
% }
% \label{tab:experiments}
% \end{table*}

==> 7--Significance_Test.tex <==
To verify the effectiveness of VIM, we adopt a paired t-test that shows how much the method affects the results. We compared the results of \llamaicl~and \villm~on value survey, behavior prediction, and opinion prediction tasks. For the value survey and opinion prediction tasks, \villm's improvement over \llamaicl~is statistically significant (p-value < 0.001). For the behavior prediction task, it varied by value; the improvement was statistically significant for Achievement and Self-direction (p-value <= 0.001), but no significance was found for the other values.


==> Table/table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% % \begin{adjustbox}{max width=\textwidth}
% \centering
% \begin{tabular}{cc|rrrrr}
% \hline
% \multicolumn{2}{c|}{\multirow{2}{*}{Model}}                                                                               & \multicolumn{5}{c}{NMSE}                                                                                                                                                                                   \\ \cline{3-7} 
% \multicolumn{2}{c|}{}                                                                                                     & \multicolumn{1}{c|}{ESS-MST} & \multicolumn{1}{c|}{ESS-PSWB} & \multicolumn{1}{c|}{ESS-POL} & \multicolumn{1}{c|}{ESS-SWB} & \multicolumn{1}{c}{ESS-UD} \\ \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Prompt\\ Based\end{tabular}}} & LLAMA-7B                     & \multicolumn{1}{r|}{0.08}                   & \multicolumn{1}{r|}{0.11}                           & \multicolumn{1}{r|}{0.28}     & \multicolumn{1}{r|}{0.28}                  & 0.07                                        \\ \cline{2-7} 
% \multicolumn{1}{c|}{}                                                                        & ChatGPT                    & \multicolumn{1}{r|}{0.22}                   & \multicolumn{1}{r|}{0.13}                           & \multicolumn{1}{r|}{\textbf{0.11}}     & \multicolumn{1}{r|}{\textbf{0.09}}                  & 0.22                                        \\ \hline
% \multicolumn{1}{c|}{\multirow{3}{*}{Ours}}                                                   & Argument Gen              & \multicolumn{1}{r|}{0.11}                   & \multicolumn{1}{r|}{0.08}                           & \multicolumn{1}{r|}{0.27}     & \multicolumn{1}{r|}{0.55}                  & 0.24                                        \\ \cline{2-7} 
% \multicolumn{1}{c|}{}                                                                        & Question Ans               & \multicolumn{1}{r|}{0.07}                   & \multicolumn{1}{r|}{0.07}                           & \multicolumn{1}{r|}{0.21}     & \multicolumn{1}{r|}{0.27}                  & \textbf{0.05}                                        \\ \cline{2-7} 
% \multicolumn{1}{c|}{}                                                                        & Argument Gen + Question Ans & \multicolumn{1}{r|}{\textbf{0.06}}                   & \multicolumn{1}{r|}{\textbf{0.06}}                           & \multicolumn{1}{r|}{0.14}     & \multicolumn{1}{r|}{0.27}                  & 0.15                                        \\ \hline
% \end{tabular}
% % \end{adjustbox}
% \caption{European Social Survey, Normalized MSE}
% \label{tab:my-table}
% \end{table*}
